Starting Small -- Learning with Adaptive Sample Sizes

For many machine learning problems, data is abundant and it may be prohibitive to make multiple passes through the full training set. In this context, we investigate strategies for dynamically increasing the effective sample size, when using iterative methods such as stochastic gradient descent. Our interest is motivated by the rise of variance-reduced methods, which achieve linear convergence rates that scale favorably for smaller sample sizes. Exploiting this feature, we show -- theoretically and empirically -- how to obtain significant speed-ups with a novel algorithm that reaches statistical accuracy on an $n$-sample in $2n$, instead of $n \log n$ steps.

==> table.tex <==

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\caption{Comparison of \methodname{} against various optimization methods in terms of suboptimality on the empirical risk and the expected risk after a single pass over the data as well as the time complexity to reach statistical $\bound\left(n\right)$-optimality. Here $\kappa$ is the condition number of the empirical risk, while
$\hat{\kappa}$ denote the condition number of the expected risk, which is used in the analysis of {\sc
SSVRG}. We used a constant step-size $\eta$ for $\eta$-SGD and a decreasing
step-size
$\eta = \frac{0.3}{0.3 + \mu t}$ for SGD . Note that all the bounds in this
table are up to constant factors; the Big O notation was left out for
simplicity. \highlight{@Aurelien: Please check caption and sgd convergence
rate}}
\label{table:convergence_comparison}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr} 
\hline
\abovespace\belowspace
 Method & Empirical Risk Suboptimality & Expected Risk Suboptimality
 & Time to reach $\bound(n)$-optimality
\\
\hline
\abovespace
SAGA   & $\exp\left(-1\right) \initerror$ & $\exp\left(-1\right) \initerror +
\frac{1}{n}$ & $n \log (\initerror n ) d$
\\
$\eta$-SGD & $ (1-2\eta\mu)^t \initerror + \frac{\eta
	\sigma^2 L}{2 \mu	}$ & $(1-2\eta\mu)^t \initerror + \frac{\eta
	\sigma^2 L}{2 \mu	} + \frac{1}{n} $& $\kappa \sigma^2
n \log(n \initerror) d$\\
SGD    & $\frac{\vartheta\kappa^2 }{n} \initerror$  & $\frac{ \vartheta\kappa^2
}{n} \initerror$ & $\kappa^2 \vartheta n d $ 
\\
SSVRG  &
\highlight{$\kappa\left(\frac{1}{n}+ \left(\frac{\kappa}{n}\right)^{1.5} \initerror
\right)$} & $\hat{\kappa}\left(\frac{1}{n}+
\left(\frac{\hat{\kappa}}{n}\right)^{1.5} \initerror \right)$ & $\left(n^{\frac{2}{3}}
\hat{\kappa}^{\frac{5}{3}} \initerror^{\frac{2}{3}} +   \hat{\kappa} n \right) d
$
\\
$\eta$-SVRG/SGD & $\frac{1}{\sqrt{n}} + \eta $ & $\frac{1}{\sqrt{n}} + \eta $ & $(n + \kappa)\log(n) d$\\
\belowspace
\textbf{\methodname}    & $
\frac{1}{n} +\left(\frac{\kappa}{n}\right)^2 \initerror$ & $
\frac{1}{n}+\left(\frac{\kappa}{n}\right)^2\initerror$ & $\left(n +
\kappa\sqrt{n \initerror}\right) d $ 
\\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
